TokenCompose: Text-to-Image Diffusion with Token-level Supervision

We present TokenCompose, a Latent Diffusion Model for text-to-image generation that achieves enhanced consistency between user-specified text prompts and model-generated images. Despite its tremendous success, the standard denoising process in the Latent Diffusion Model takes text prompts as conditions only, absent explicit constraint for the consistency between the text prompts and the image contents, leading to unsatisfactory results for composing multiple object categories. TokenCompose aims to improve multi-category instance composition by introducing the token-wise consistency terms between the image content and object segmentation maps in the finetuning stage. TokenCompose can be applied directly to the existing training pipeline of text-conditioned diffusion models without extra human labeling information. By finetuning Stable Diffusion, the model exhibits significant improvements in multi-category instance composition and enhanced photorealism for its generated images. Project link: https://mlpc-ucsd.github.io/TokenCompose

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{sidecap,wasysym,array,tabularx,caption}
% \usepackage{wrapfig,lipsum,booktabs}


% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}

% \definecolor{A4B1}{RGB}{44,149,150}
% \definecolor{mTry}{RGB}{135,35,64}
% \definecolor{vEqu}{RGB}{134,74,249}
% \definecolor{newblue}{RGB}{48,48,255}



% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% \definecolor{cello}{HTML}{f2ffea}

% \definecolor{lightblue}{HTML}{e1f4ff}
% \newcommand{\colorlightblue}{\colorbox{lightblue}}
% \newcommand{\cellcolorlightblue}{\cellcolor{lightblue}}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \usepackage[subtle,charwidths=tight]{savetrees}

% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% \setcounter{figure}{0}
% \renewcommand{\figurename}{Fig.}
% \renewcommand{\thefigure}{R\arabic{figure}}

% \setcounter{table}{0}
% \renewcommand{\tablename}{Table}
% \renewcommand{\thetable}{R\arabic{table}}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{10391} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}



% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{\LaTeX\ Guidelines for Author Response}  % **** Enter the paper title here

% % \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW

% \noindent We thank all reviewers for the constructive feedback! We provide responses below and will update our manuscript accordingly.

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{mTry}{mTry})} Preservation of physical rules.}} Thanks for your question. More visualizations provided in Fig. \ref{fig:phys_rules_aggr} show that object affordance (e.g., attach, sit, support, \textit{etc}) can be maintained, which indicates that TokenCompose is able to implicitly learn the basic ``physical rules'' via the object token and segmentation consistency constraints. Failure cases shown in Fig. \ref{fig:fail_case_analysis} show that feature-level inconsistency is sometimes observed with objects, though basic physics is still somewhat obeyed.

% \begin{figure}[h]
%   \centering
%   \vspace{-2ex}
%   \includegraphics[width=1\linewidth]{figures/phys_rules_aggr.pdf}
%   \vspace{-5ex}
%    \caption{\small{More samples} in multi-category instance composition.}
%    \label{fig:phys_rules_aggr}
%    \vspace{-3ex}
% \end{figure}

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{mTry}{mTry})} Downstream applications.}} Thanks. Following your suggestions, we show in Fig. \ref{fig:downstream_apps} positive impacts in downstream applications. As expected, TokenCompose shows its effectiveness in tasks beyond text-to-image generation, \emph{including image editing, inpainting, and outpainting}.
% %Our method makes downstream apps more accessible when prompts involve \textbf{similar objects} or \textbf{being complex}, which is often the case in real-world usage.

% \begin{figure}[h]
% \vspace{-2.3ex}
%   \centering
%   \includegraphics[width=1\linewidth]{figures/downstream_apps.pdf}
%   \vspace{-5.1ex}
%    \caption{Results on image editing, outpainting, and inpainting.}
%    \label{fig:downstream_apps}
%    \vspace{-3ex}
% \end{figure}

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{A4B1}{A4B1})} Incremental novelty advancement.}} We acknowledge your perspective. \emph{Training cross-attention activation itself and its outcome} have rarely been explored or experimented with in previous literature. With the recipe and the positive results we have, we hope that our contributions can spark more fine-grained training explorations in improving compositional generation of text-to-image models.

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{A4B1}{A4B1})} Generation quality degradation due to mask quality.}} Thanks. The improvements in image quality for having grounding 
% \setlength{\columnsep}{2pt}%
% \begin{wraptable}[4]{l}{0.35\linewidth} 
% \centering 
% \resizebox{\linewidth}{!}{
% % \vspace{2ex}
%  \raisebox{0pt}[\dimexpr\height-1.6\baselineskip\relax]{\begin{tabular}{l|ll}
% \hline
% \toprule
% Model  & ft. w. & ft. w.o. \\
%  & masks & masks \\
% \midrule
% SD 1.4 & \textbf{20.19}               & 23.04                 \\
% SD 2.1 & \textbf{19.15}               & 20.55                \\
% \bottomrule
% \hline
% \end{tabular}}
% % \vspace{-3pt}
% }
% \end{wraptable}
% objectives during training outweigh possible degradation due to the quality of model-generated masks, which we show in terms of FID scores (lower is better), a simplified version of Table 2 and 3 from the main paper.

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{vEqu}{vEqu} \& \textcolor{A4B1}{A4B1})} Poor performance categories \& failure analysis.}} Thanks. We provide generated and detected samples for hard and easy categories in Fig. \ref{fig:succ_rate_exp}. We believe that one explanation for the poor performance categories is that images of these categories have \emph{variants and viewpoints with drastic visual differences}, so learning and generating them is harder. Further, we aggregate patterns of common failures in our multi-category instance composition in Fig. \ref{fig:fail_case_analysis}. We believe that visual commonsense reasoning aspect of the generative model would be an area of improvement.


% \noindent \textcolor{newblue}{\textit{\textbf{(\textcolor{vEqu}{vEqu})} Comparison \& discussion w. other relevant works.}} Thanks for the references. Masks used in RAPHAEL are generated based on the activation of model's cross-attention to assign different image regions to different experts. The masks in our setting are \emph{part of the data} to \emph{supervise the activation of cross-attention}. ERNIE-ViLG 2.0 uses \emph{a weighted denoising loss} based on regions with objects. The denoising loss is not calculated token-wise. DiffuMask adopts a Stable Diffusion (SD) model to generate semantic segmentation maps. Notably, they mention, ``\textit{In our experiment, only a single object for an image is considered. Multi-categories generation usually causes the unstable quality of the images, limited by the generation ability of Stable Diffusion,}" echoing the potential of our contributions. VPD is less impacted by compositionality issues as their tasks do not involve denoising from noise but real images, a setting not applicable for generation. We'll include them in addition to P2P following your suggestions.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/succ_rate_compare.pdf}
%   \vspace{-5ex}
%    \caption{\small{Categories with poor \& strong performance.}}
%    \label{fig:succ_rate_exp}
%    \vspace{-2ex}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/failure_case_analysis.pdf}
%   \vspace{-4.75ex}
%    \caption{\small{Failure case analysis in multi-category  compositionality.}}
%    \label{fig:fail_case_analysis}
%    \vspace{-4.75ex}
% \end{figure}

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{vEqu}{vEqu})} Comparison with models using the T5 encoder.}} Thanks. PixArt-$\alpha$ with the T5 encoder brings better compositional capabilities as shown in the upper Table \ref{tab:pixart_numbers}. Finetuning SD with our objective yields superior performance on VISOR, MG-COCO and on-par performance on MG-ADE20K despite more than $10\times$ text encoder size difference, as shown in the lower Table \ref{tab:pixart_numbers}. Qualitatively, we still observe that PixArt-$\alpha$ misses or mixes objects in Fig. \ref{fig:pixart_failures}, indicating (1) a stronger text encoder alone does not \emph{eliminate} compositional issues, and (2) using fine-grained training objectives may further improve PixArt-$\alpha$'s compositional performance.

% \vspace{-2ex}
% \begin{table}[h]
% \centering
% \scalebox{0.585}{
% \begin{tabular}{lcc|c|ccc|ccc@{}}
% \hline
% \toprule

% \textbf{Model} & \textbf{Enc$_\text{text}$} & \textbf{\# Enc$_\text{text}$} & \textsc{} & \multicolumn{3}{c|}{\textsc{MG} (COCO)} & \multicolumn{3}{c}{\textsc{MG} (ADE20K)}  \\

%  & & \textbf{Params} & OA & MG3 & MG4 & MG5 & MG3 & MG4 & MG5\\

% \midrule
% SD 1.4 & CLIP-ViT/L & 0.12B & 29.86  & 50.74 & 11.68 & 0.88 & 53.96 & 16.52 & 1.89 \\
% SD 2.1 & OpenCLIP-ViT/H & 0.34B & 47.82 & 70.14 & 25.57 & 3.27 & 75.13 & 35.07 & 7.16 \\

% PixArt-$\alpha$ & Flan T5 XXL & 4.3B & 49.53& 75.96 & 31.35 & 4.91 & \textbf{81.42} & \textbf{41.66} & \textbf{8.86} \\
% \midrule
% \multicolumn{3}{c|}{\emph{\textbf{Ours}} (ft. w. $\mathcal{L}_{\text{pixel}}$ and $\mathcal{L}_{\text{token}}$) }  & & & & \\
% SD 1.4 & CLIP-ViT/L & \underline{\textbf{0.12B}} & \underline{52.15} & \underline{76.16} & 28.81 & 3.28 & 76.93 & 33.92 & 6.21 \\
% SD 2.1 & OpenCLIP-ViT/H & \underline{0.34B} & \underline{\textbf{60.10}} &  \underline{\textbf{80.48}} & \underline{\textbf{36.69}} & \underline{\textbf{5.71}} & 79.51 & 39.59 & 8.13\\

% \bottomrule
% \hline
% \end{tabular}
% }
% \vspace{-1.6ex}
% \caption{Comparison with PixArt-$\alpha$. Best numbers are \textbf{bolded}, and numbers better than the PixArt-$\alpha$ baseline are \underline{underlined}.} 
% \label{tab:pixart_numbers}
% \vspace{-3ex}
% \end{table}

% \begin{figure}[h]
% \vspace{-2ex}
%   \centering
%   \includegraphics[width=1\linewidth]{figures/pixart_failures.pdf}
%   \vspace{-4.5ex}
%    \caption{\small{\textcolor[RGB]{255, 1, 0}{Red}: \emph{missed} obj.; \textcolor[RGB]{233, 133, 50}{Orange}: \emph{mixed} obj.; \textcolor[RGB]{8, 178, 85}{Green}: generated obj.}}
%    \label{fig:pixart_failures}
% \end{figure}
% \vspace{-2.5ex}
% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{vEqu}{vEqu})} Confused title.}} Thanks for your suggestion! We will replace the term ``\emph{grounding}" with ``\emph{text-to-image}" from the title.

% \noindent\textcolor{newblue}{\textit{\textbf{(\textcolor{vEqu}{vEqu})} Open-source availability.}} Weights for detectors in both works are available on HuggingFace prior to submission and can be readily used with the \texttt{transformers} package.

% \end{document}


==> sup_submit.tex <==
% % CVPR 2024 Paper Template; see https://github.com/cvpr-org/author-kit

% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% \usepackage{cvpr}              % To produce the CAMERA-READY version
% % \usepackage[review]{cvpr}      % To produce the REVIEW version
% % \usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % It is strongly recommended to use hyperref, especially for the review version.
% % hyperref with option pagebackref eases the reviewers' job.
% % Please disable hyperref *only* if you encounter grave issues, 
% % e.g. with the file validation for the camera-ready version.
% %
% % If you comment hyperref and then uncomment it, you should delete *.aux before re-running LaTeX.
% % (Or just hit 'q' on the first LaTeX run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}
% \usepackage{xcolor,colortbl}
% \usepackage{multirow}
% \usepackage{array,booktabs}
% \usepackage{placeins}
% \usepackage{amsmath}
% \usepackage[normalem]{ulem}
% % \usepackage{scalerel,graphicx,xparse}
% % \NewDocumentCommand\emojione{}{\scalerel*{\includegraphics{1F44F}}{X}}
% \usepackage{hwemoji}
% \usepackage{wasysym}
% \usepackage{float}
% \usepackage{sidecap}
% % \usepackage{coloremoji}
% % \usepackage{multicol}


% \usepackage{algorithm,algorithmicx,algpseudocode}

% \newcolumntype{C}{>{$\displaystyle}c<{$}}

% \definecolor{citecolor}{HTML}{0b64c5}

% % change the color for better visual consistency
% \definecolor{cello}{HTML}{f2ffea}
% \newcommand{\colorcello}{\cellcolor{cello}}

% \definecolor{lightblue}{HTML}{e1f4ff}
% \newcommand{\colorlightblue}{\colorbox{lightblue}}
% \newcommand{\cellcolorlightblue}{\cellcolor{lightblue}}

% \definecolor{lightgray}{HTML}{f2f2f2}
% \newcommand{\colorlightgray}{\colorbox{lightgray}}
% \newcommand{\cellcolorlightgray}{\cellcolor{lightgray}}

% \definecolor{lightpurple}{HTML}{f2eaff}
% \newcommand{\colorlightpurple}{\colorbox{lightpurple}}
% \newcommand{\cellcolorlightpurple}{\cellcolor{lightpurple}}

% \definecolor{lightgreen}{HTML}{f2ffea}
% \newcommand{\colorlightgreen}{\colorbox{lightgreen}}
% \newcommand{\cellcolorlightgreen}{\cellcolor{lightgreen}}

% \definecolor{sp_lightgreen}{HTML}{e2f0d9}
% \newcommand{\colorsplightgreen}{\colorbox{sp_lightgreen}}
% \newcommand{\cellcolorsplightgreen}{\cellcolor{sp_lightgreen}}

% \definecolor{sp_lightorange}{HTML}{fbe5d6}
% \newcommand{\colorsplightorange}{\colorbox{sp_lightorange}}
% \newcommand{\cellcolorsplightorange}{\cellcolor{sp_lightorange}}

% \newcommand{\cw}[1]{\textcolor{red}{[cw: #1]}}

% \newcommand{\szz}[1]{\textcolor{blue}{[szz: #1]}}

% \definecolor{lblue}{rgb}{0.2, 0.5, 0.9}
% \newcommand{\zheng}[1]{{\color{lblue} [zheng: #1]}}

% \makeatletter
% \@addtoreset{section}{part}
% \def\@part[#1]#2{%
%     \ifnum \c@secnumdepth >\m@ne
%       \refstepcounter{part}%
%       \addcontentsline{toc}{part}{\thepart\hspace{1em}#1}%
%     \else
%       \addcontentsline{toc}{part}{#1}%
%     \fi
%     {\parindent \z@ \raggedright
%      \interlinepenalty \@M
%      \normalfont\centering
%      \ifnum \c@secnumdepth >\m@ne
%        \LARGE\bfseries \partname\nobreakspace\thepart
%        \par\nobreak
%      \fi
%      \huge \bfseries #2%
%      \markboth{}{}\par}%
%     \nobreak
%     \vskip 3ex
%     \@afterheading}
% \renewcommand\partname{Topic}
% \makeatother

% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{10391} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}

% % this error needs to be fixed
% \DeclareUnicodeCharacter{1EAF}{\'a}


% %%%%%%%%% TITLE - PLEASE UPDATE
% % \title{Steering Diffusion toward Instance Awareness}
% % \title{Learning Discrimination via Generation in Diffusion Models}
% \title{\textsc{TokenCompose}: Text-to-Image Diffusion with Token-level Supervision}
% %%%%%%%%% AUTHORS - PLEASE UPDATE
% \author{%
%   Zirui Wang$^{\clubsuit,\spadesuit}$ \qquad Zhizhou Sha$^{\vardiamond,\spadesuit}$ \qquad Zheng Ding$^{\spadesuit}$ \qquad
%   Yilin Wang$^{\vardiamond,\spadesuit}$ \qquad Zhuowen Tu$^{\spadesuit}$ \\
%   %
%   $^\clubsuit$Princeton University \qquad $^\vardiamond$Tsinghua University \qquad $^\spadesuit$University of California, San Diego \\
%   \url{https://mlpc-ucsd.github.io/TokenCompose}
% }

% \begin{document}

% \input{commands}

% % WARNING: do not forget to delete the supplementary pages from your submission 

% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary

% \section{Pipeline Setup}
% \label{sec:pipeline_details}
% We provide detailed data generation, training and inference settings for the \textsc{TokenCompose} pipeline setup in Table \ref{tab:pipeline_param}. Unless otherwise specified, experiments are run based on this set of settings. For settings that are not reported in Table \ref{tab:pipeline_param}, we follow the default values provided by their respective codebases.

% \begin{table}[hb!]
% \centering
% \vspace{-2ex}
% \scalebox{0.92}{
% \begin{tabular}{l|l}
% \hline
% % header
% \toprule
% \multicolumn{1}{l}{\multirow{-1}{*}{\textbf{Setting}}} & \textbf{Value} \\

% \midrule
% \textbf{\emph{Data Generation}} \\
% \quad \small CLIP Model & \small \texttt{ViT-L/14@336px} \cite{clip, vit} \\
% \quad \small POS Tagger & \small \texttt{flair/pos-english} \cite{flair} \\
% \quad \small Target POS Tags & \small NN / NNS / NNP / NNPS \\
% \quad \small G. DINO Model & \scriptsize \texttt{groundingdino\_swint\_ogc} \small \cite{grounding_dino, dino, swin} \\
% \quad \small G. DINO Box Thres. & 0.25 \\
% \quad \small G. DINO Text Thres. & 0.25 \\
% \quad \small SAM Model & \small \texttt{sam\_hq\_vit\_h} \cite{vit, sam, sam_hq} \\

% \textbf{\emph{Training}} \\
% \quad \small Resolution \textsubscript{SD 1.4} & \small $512 \times 512$ \\
% \quad \small Resolution \textsubscript{SD 2.1} & \small $768 \times 768$ \\
% \quad \small Image Processing & \small Center Crop + Resize \\
% \quad \small Batch Size & \small 1 \\
% \quad \small Grad. Accum. Steps & \small 4 \\
% \quad \small Grad. Ckpting. & \small \texttt{True} \\
% \quad \small Train Steps \textsubscript{SD 1.4} & \small 24000 \\
% \quad \small Train Steps \textsubscript{SD 2.1} & \small 32000 \\
% \quad \small Learning Rate & \small 5e-6 \\
% \quad \small LR Scheduler & \small Constant \\
% \quad \small LR Warmup & \small \texttt{False} \\
% \quad \small $\lambda$ for $\mathcal{L}_{token}$ & \small 1e-3 \\
% \quad \small $\gamma$ for $\mathcal{L}_{pixel}$ & \small 5e-5 \\
% \quad \small $\mathcal{L}_{token}$ and $\mathcal{L}_{pixel}$ & all layers in $U_{\text{Mid}}$ and $U_{\text{D}}$ \\
% \quad \small Clf-Free Guidance \cite{classifier_free_guidance} & \small \texttt{False} \\

% \textbf{\emph{Inference}} \\
% \quad \small Resolution \textsubscript{SD 1.4} & \small $512 \times 512$ \\
% \quad \small Resolution \textsubscript{SD 2.1} & \small $768 \times 768$ \\
% \quad \small Timestep Scheduler & \small \texttt{PNDMScheduler} \\
% \quad \small \# Inference Steps & \small 50 \\
% \quad \small Clf-Free Guidance \cite{classifier_free_guidance} & \small \texttt{True} \\
% \quad \small Guidance Scale & \small 7.5 \\


% \bottomrule
% \hline
% \end{tabular}
% }
% \vspace{-2ex}
% \caption{\textbf{Model choices and settings for data generation, training, and inference.} We provide a comprehensive list of pipeline details for data generation (\textit{e.g.,} caption selection, noun extraction and segmentation map generation), training (\textit{e.g.,} finetuning the Stable Diffusion model), and inference (\textit{e.g.,} evaluation of our finetuned Stable Diffusion model).}
% \label{tab:pipeline_param}
% \vspace{-4ex}
% \end{table}

% \section{Conditional Downstream Metrics}

% \begin{figure}[ht!]
%   \centering
%     \includegraphics[width=1\linewidth]{figures/conditioned_t2i_bench.pdf}
%     \vspace{-4ex}
%     \caption{\textbf{Improvement comparison of unconditional and conditional downstream compositional metrics.} We illustrate that a significant margin of downstream compositional metrics is improved due to enhanced capabilities of multi-category instance composition. In this figure, we calculate the evaluation metrics from T2I-CompBench \cite{t2i_bench} by conditioning on the successful generation of all instances mentioned in the prompts, and compare the amount of quantitative improvement with the same metrics that are \emph{not} conditioned on successfull generation of all instances.}
%     \label{fig:conditioned_metrics}
% \vspace{-4ex}
% \end{figure}

% As multi-category instance composition serves as a prerequisite for successful downstream text-conditioned compositional generation, we conjecture that the improvements in downstream metrics are improved by higher chances of generating all instances mentioned in the prompt. In this section, we provide an additional object accuracy metric in Table \ref{tab:oa_t2i_bench}, and show that \textsc{TokenCompose} improves object accuracy in all downstream metrics being evaluated. Furthermore, in Figure \ref{fig:conditioned_metrics}, we demonstrate how better multi-category instance composition capabilities can improve these metrics by plotting the improvement curve from \textbf{\emph{(1)}} a frozen Stable Diffusion to \textbf{\emph{(2)}} a Stable Diffusion finetuned with only $\lsimplelcm$ objective, and finally to \textbf{\emph{(3)}} a Stable Diffusion model finetuned with both $\lsimplelcm$ and our grounding objectives conditioned and unconditioned on successful generation of all instances from the compositional prompts. 

% From the results, we observe that the improvements in all attribute binding metrics (\textit{e.g.,} color, shape, texture) and the majority of object relation metrics (\textit{e.g.,} spatial, complex) are much more significant in the unconditional case than in the conditional case. The only downstream benchmark where the difference in improvement is insignificant is the \emph{non-spatial} compositionality. We believe that this insignificance can be explained by two factors: (1) lowest amount of improvement in object accuracy for this specific downstream benchmark, as shown in Table \ref{tab:oa_t2i_bench} and (2) relatively low correlation between automatic scores (\textit{i.e.,} CLIP Score \cite{clip, clip_score}) and human ratings among all compositional benchmarks from the T2I-CompBench \cite{t2i_bench}; this indicates that the evaluation model may have a comparably weak discriminative capability for this specific task.

% \begin{table}[ht]
% \centering
% \scalebox{0.75}{
% \begin{tabular}{l|cccccc}
% \hline
% % header
% \toprule
% \multicolumn{1}{l}{\multirow{-1}{*}{\textbf{Model}}} & \small Color & \small Shape & \small Texture & \small Spatial & \small Non-Spat. & \small Complex \\

% \midrule
% \textbf{\emph{SD 1.4}} \\
% \quad frozen & 47.40 & 25.33 & 15.27 & 19.40 & 45.10 & 26.60  \\
% \quad ft. w. \small $\lsimplelcm$ & 55.70 & 28.49 & 18.95 & 27.05 & 47.33 & 29.33 \\
% \midrule
% \colorcello \quad \emph{\textbf{Ours}} & \colorcello \textbf{62.92} & \colorcello \textbf{32.95} & \colorcello \textbf{25.59} & \colorcello \textbf{33.30} & \colorcello \textbf{48.94} & \colorcello \textbf{32.10} \\

% \bottomrule
% \hline
% \end{tabular}
% }
% \vspace{-2ex}
% \caption{\textbf{Object accuracy in downstream compositional metrics.} We calculate the object accuracy metric (\textit{i.e.,} success rate of generating all instances in the prompt based on a detection model \cite{owlv2}) for each of the compositional benchmarks from T2I-CompBench \cite{t2i_bench}.}
% \label{tab:oa_t2i_bench}
% \vspace{-2ex}
% \end{table}

% \begin{figure}[ht]
%   \centering
%   \vspace{-0.5ex}
%     \includegraphics[width=1\linewidth]{figures/dataset_metadata.pdf}
%     \vspace{-4ex}
%     \caption{\textbf{Approximations of the average number of tokens with grounding objectives per training prompt.} From left to right, we show the distribution of number of tokens per caption, number of noun tokens per caption, and number of noun tokens that have generated segmentation maps per caption.}
%     \label{fig:dataset_metadata}
% \vspace{-3ex}
% \end{figure}

% \begin{figure*}[ht]
%   \centering
%   \vspace{-2ex}
%   \includegraphics[width=1\linewidth]{figures/phys_rules_aggr.pdf}
%   \vspace{-4ex}
%    \caption{\textbf{More samples} in multi-category instance composition.}
%    \label{fig:phys_rules_aggr}
% \end{figure*}

% \begin{figure*}[ht]
%   \centering
%   \vspace{-2ex}
%   \includegraphics[width=1\linewidth]{figures/downstream_apps.pdf}
%   \vspace{-5ex}
%    \caption{\textbf{Downstream applications} in prompt-to-prompt \cite{hertz2022prompt} image editing and zero-shot outpainting and inpainting.}
%    \label{fig:downstream_apps}
% \end{figure*}

% \begin{figure*}[ht!]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/succ_rate_compare.pdf}
%   \vspace{-5ex}
%    \caption{Categories with poor \& strong performance}.
%    \label{fig:succ_rate_exp}
%    \vspace{-2ex}
% \end{figure*}

% \begin{figure*}[ht!]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/failure_case_analysis.pdf}
%   \vspace{-5ex}
%    \caption{\textbf{Failure case analysis} in multi-category compositionality.}
%    \label{fig:fail_case_analysis}
%    \vspace{-2ex}
% \end{figure*}



% \begin{figure*}[ht!]
%   \centering
%     \includegraphics[width=1\linewidth]{figures/multigen_viz.pdf}
%     % \vspace{-5ex}
%     \caption{\textbf{Sampled images with prompts from our \textsc{MultiGen} benchmark.} To facilitate understanding of our multi-category instance composition benchmark as well as further qualitative comparisons among different baselines, we provide sampled images from \textsc{MultiGen} with COCO instances as well as ADE20K instances.}
%     \label{fig:multigen_viz}
% \vspace{-2ex}
% \end{figure*}

% \begin{figure*}[ht!]
%   \centering
%     \includegraphics[width=1\linewidth]{figures/dataset_vis.pdf}
%     % \vspace{-5ex}
%     \caption{\textbf{Grounding dataset visualization.} We provide visualizations of 50 selected image-text pairs (number of noun tokens with segmentation maps $\geq 5$) and their corresponding token-level binary segmentation maps from the training data to facilitate understanding of our training dataset.}
%     \label{fig:dataset_vis}
% \vspace{+4ex}
% \end{figure*}

% \section{More Examples}
% \textbf{Multi-category Instance Composition.} We provide more visualizations in Figure. \ref{fig:phys_rules_aggr} to illustrate capabilities of TokenCompose in multi-category instance composition. In addition to being able to generate multiple categories of instances successfully, we show that object affordance (\textit{e.g.,} attach, sit, support, \textit{etc}) can be maintained, which indicates that TokenCompose is able to implicitly learn the basic ``physical rules" via the object token and segmentation consistency constraints. 

% \textbf{Downstream Applications.} We show in Figure. \ref{fig:downstream_apps} positive impacts in downstream applications. As expected, TokenCompose shows its effectiveness in tasks beyond text-to-image generation.

% \textbf{Benchmark.} \textsc{MultiGen} benchmark plays a crucial role in evaluating multi-category instance composition capabilities of text-to-image models. To offer a more intuitive sense in this compositional task, we visualize the generated images from various prompts in this benchmark (\textit{e.g.,} MG COCO Instances and MG ADE20K Instances). We use the same latent for each comparison for fairness. The images are presented in Figure \ref{fig:multigen_viz}.

% \section{Grounded COCO Dataset}
% As seen in Figure 2 from the main paper, we adopt a POS Tagger and the Grounded SAM \cite{flair, grounding_dino, sam} to extract binary segmentation maps from noun tokens from the image-text pair dataset. We aim to expand the visualizations of the generated data in Figure \ref{fig:dataset_vis}. Each row and column represents a single data that the model is trained with. From the left to the right of the data are the caption, the input image, and the grounded binary segmentation maps. 

% The bold and underlined \underline{\textbf{text}} in the caption represents noun tokens captured by the POS tagger where their corresponding segmentation maps are extracted from the Grounded SAM. Italicized and red \textcolor{red}{\textit{text}} in the caption represents noun tokens captured by the POS tagger but does \emph{not} have segmentation maps extracted from the Grounded SAM due to the model not being able to locate the objects.

% Grounded segmentation maps on the right are paired with their correpsonding tokens. For tokens with a green \colorbox{sp_lightgreen}{background}, their segmentation maps successfully capture the aligned contents in the image, whereas for a small fraction of tokens with an orange \colorbox{sp_lightorange}{background}, their segmentation maps do not capture the aligned contents in the image.

% We also provide reference on approximations (\textit{i.e.,} word split by space) of (1) average number of tokens per caption, (2) average number of \emph{noun tokens} per caption, and (3) average number of noun tokens that \emph{have their corresponding segmentation maps} per caption in Figure \ref{fig:dataset_metadata}. As shown in the figure, our training dataset contains an average of 3.71 noun tokens overall and 3.21 noun tokens that have their corresponding segmentation maps.

% \section{Analysis}

% \textbf{Attention Visualizations.} To gain a better understanding of how incorporating grounding objectives into text-to-image models during training affects cross-attention maps for image reconstruction \cite{null_text_inversion} \& generation tasks at inference time, we provide token-level cross-attention map visualizations on three axes: \emph{\textbf{(1)}} different cross-attention layers with various resolutions (Figure \ref{fig:ca_by_res}); \emph{\textbf{(2)}} different heads of the multi-head cross-attention (Figure \ref{fig:ca_by_head}; and \emph{\textbf{(3)}} different timesteps during the denoising process (Figure \ref{fig:ca_by_timestep}).

% \textbf{Multi-category Instance Composition Success Rate.} 
% Given a set of compositional prompts, we calculate the count of each category that appears in these prompts along with images where the instance(s) of this category is/are detected by a detection model \cite{owlv2}. We divide the number of images that contain a specific category of the instance by the number of prompts that contains this category to acquire the success rate and report the numbers in Figure \ref{fig:success_rate}.

% \textbf{Failure Cases.} 
% We provide generated and detected samples for categories with low and high success rates in Figure. \ref{fig:succ_rate_exp}. We believe that one explanation for the poor performance categories have variants and viewpoints with drastic visual differences, so learning and generating them is harder. Further, we aggregate patterns of common failures in our multi-category instance composition in Figure. \ref{fig:fail_case_analysis}. We believe that visual commonsense reasoning aspect of the generative model would be an area of improvement.

% \begin{figure*}[ht!]
%   \centering
%     \includegraphics[width=0.95\linewidth]{figures/ca_by_res.pdf}
%     % \vspace{-5ex}
%     \caption{\textbf{Cross-attention map visualizations by different cross-attention layers at denoising U-Net.} We visualize the cross-attention map between a frozen Stable Diffusion \cite{ldm} model and our model at the middle block and decoder layers of the denoising U-Net, where cross-attention at these layers are trained with our grounding objectives. In the upper example, we leverage null text inversion \cite{null_text_inversion} to let two models reconstruct similar images using different latents for comparable cross-attention maps to demonstrate stronger grounding capabilities of our model. In the lower example, we use the same initial latent for two different models to generate images to demonstrate how stronger grounding capabilities lead to better compositionality.}
%     \label{fig:ca_by_res}
% \vspace{-4ex}
% \end{figure*}

% \begin{figure*}[ht!]
%   \centering
%     \includegraphics[width=1\linewidth]{figures/ca_by_head.pdf}
%     % \vspace{-5ex}
%     \caption{\textbf{Cross-attention map visualizations by different cross-attention heads at the denoising U-Net.} We visualize the cross-attention map of each head at the last layer (\textit{i.e.,} $U_{\text{D}}^{64 \times 64}$) of the U-Net decoder between a frozen Stable Diffusion \cite{ldm} model and our model. We use the same setting as in Figure \ref{fig:ca_by_res} but with a different prompt for a more diverse visualization. We show that our grounding objective \emph{allows} flexibility of different heads to attend to different regions of the latent.}
%     \label{fig:ca_by_head}
% \vspace{-4ex}
% \end{figure*}

% \begin{figure*}[ht!]
%   \centering
%     \includegraphics[width=0.9\linewidth]{figures/ca_by_timestep.pdf}
%     % \vspace{-5ex}
%     \caption{\textbf{Cross-attention map visualizations by different denoising time steps at the denoising U-Net.} We visualize the cross-attention map of the last layer (\textit{i.e.,} $U_{\text{D}}^{64 \times 64}$) of the U-Net decoder between a frozen Stable Diffusion \cite{ldm} model and our model at time step 1 and every 5 steps based on a 50-step DDIM \cite{ddim} scheduler. We use the same setting as in Figure \ref{fig:ca_by_res} with a different prompt for a more diverse visualization. We show that our grounding objective enables cross-attention of different object tokens to aggregate at different regions of the noisy latent \emph{early} during inference. This enables the model to generate different categories of instances more successfully, leading to better multi-category instance composition capabilities.}
%     \label{fig:ca_by_timestep}
% \vspace{-4ex}
% \end{figure*}

% \begin{figure*}[ht!]
%   \centering
%     \includegraphics[width=1\linewidth]{figures/success_rate.pdf}
%     % \vspace{-5ex}
%     \caption{\textbf{Instance generation success rate in multi-category instance composition benchmarks.} We provide the success rate (from a 0-1 scale) of generating instances with our best-performing model for VISOR \cite{visor}, MG-COCO, and MG-ADE20K benchmarks.}
%     \label{fig:success_rate}
% \vspace{+8ex}
% \end{figure*}

% \pagebreak

% % \clearpage

% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{main}
% }
% \end{document}

